Application of Ontologies in Identifying Requirements Patterns in Use Cases

Use case specifications have successfully been used for requirements description. They allow joining, in the same modeling space, the expectations of the stakeholders as well as the needs of the software engineer and analyst involved in the process. While use cases are not meant to describe a system's implementation, by formalizing their description we are able to extract implementation relevant information from them. More specifically, we are interested in identifying requirements patterns (common requirements with typical implementation solutions) in support for a requirements based software development approach. In the paper we propose the transformation of Use Case descriptions expressed in a Controlled Natural Language into an ontology expressed in the Web Ontology Language (OWL). OWL's query engines can then be used to identify requirements patterns expressed as queries over the ontology. We describe a tool that we have developed to support the approach and provide an example of usage.

==> eptcsdata.tex <==
\providecommand{\firstpage}{62}
\providecommand{\publicationstatus}{B. Buhnova, L. Happe, J. Kofro\v n (Eds.): Formal Engineering\\
Approaches to Software Components and Architectures 2014\\
EPTCS 147, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.147.5}{10.4204/EPTCS.147.5}}
\pdfoutput=1

